Cooperative Receding Horizon 3D Coverage Control with a Team of Networked Aerial Agents

This work proposes a receding horizon coverage control approach which allows multiple autonomous aerial agents to work cooperatively in order cover the total surface area of a 3D object of interest. The cooperative coverage problem which is posed in this work as an optimal control problem, jointly optimizes the agents' kinematic and camera control inputs, while considering coupling constraints amongst the team of agents which aim at minimizing the duplication of work. To generate look-ahead coverage trajectories over a finite planning horizon, the proposed approach integrates visibility constraints into the proposed coverage controller in order to determine the visible part of the object with respect to the agents' future states. In particular, we show how non-linear and non-convex visibility determination constraints can be transformed into logical constraints which can easily be embedded into a mixed integer optimization program.

==> ack.tex <==
\section*{Acknowledgments}
This work is supported by Cyprus Research and Innovation Foundation under grant agreement EXCELLENCE/0421/0586 (GLIMPSE), by the European Union's Horizon 2020 research and innovation programme under grant agreement No 739551 (KIOS CoE), and from the Republic of Cyprus through the Directorate General for European Programmes, Coordination and Development.

==> relatedWork.tex <==
\section{Related Work}\label{sec:Related_Work}








%Initial works on coverage path planning (CPP) have mainly employed ground robots with fixed sensors for the coverage task \cite{Choset2001,Galceran2013}. The majority of these approaches \cite{Choset1998,Acar2002} usually proceed by decomposing the area of interest in a number of non-overlapping cells, and subsequently solving an optimization problem to find the robot's path that passes from all the cells, thus achieving full coverage of the area of interest. In \cite{Acar2002sensor,Batsaikhan2013} the authors propose coverage planning techniques which allow the robot to cover the region of interest while simultaneously constructing the cell decomposition, whereas in \cite{Acar2006,Huang2001,Mnnadiar2010} the coverage planning task is investigated with respect to the sweeping direction, the sensor size, and the cell traversal order. In \cite{Wong2003} the authors propose an exact cellular decomposition coverage planning approach based on the detection of natural landmarks, whereas in \cite{Gabriely2001} a spanning-tree based CPP approach is proposed for a ground robot equipped with a square-shaped sensor.
%
%The coverage planning problem has also been extended to multi-robot systems \cite{Almadhoun2019}. In \cite{Gao2018} the area of interest is divided amongst multiple robots, which then utilize ant colony optimization to obtain the coverage path of their assigned area, whereas in \cite{Sipahioglu2010} a multi-robot coverage planning approach is proposed based on the capacitated arc routing problem (CARP), in order to construct coverage paths according to the energy capacity limitations of the robots. In \cite{Rekleitis2008} a boustrophedon cellular decomposition algorithm \cite{Choset2000} is proposed for a multi-robot system with communication constraints, whereas in \cite{Janchiv2013} the problem of multi-robot coverage path planning is posed as a network flow problem, which minimizes the total coverage time. In \cite{Cannata2011}, a graph-based coverage algorithm is proposed which allows multi-robot system to repeatedly cover a set of locations according to a specified frequency distribution, whereas in \cite{Tolstaya2021} graph neural networks are employed for the problem of multi-robot coverage. 
%
%   
%More recently the coverage path planning problem has been considered for UAV-based systems and applications. The authors in \cite{Papaioannou2021a,Papaioannou2021b} propose a UAV-based 3D coverage planning approach based on mixed integer quadratic programming, which enables the generation of UAV trajectories that can be used to cover in 3D cuboid-like objects of interest. An exact cellular decomposition CPP approach for polygonal convex areas is proposed in \cite{Li2011}, whereas in \cite{Xu2014} a coverage planning approach is proposed for a fixed-wing UAV. In \cite{Xu2014} the terrain which needs to be covered with the UAV is first split into a number of non-overlapping cells. At a second stage the Chinese postman problem \cite{Pearn1995} is solved to compute an Eulerian circuit traversing through these cells. In \cite{Liam2014} the authors propose an information theoretic terrain coverage path planning approach for fixed-wing UAV, and in \cite{Chen2021} multiple heterogeneous UAVs are being utilized to search and cover multiple planar regions of interest based on their capabilities. The coverage path planning problem is also investigated in \cite{Bentz2018,Cabreira2019,Choi2020} for UAV systems which exhibit energy limitations and constraints. A multi-UAV coverage planning approach for 2D terrain coverage is also proposed in \cite{Collins2021}, which aims at minimizing the completion time by providing a balanced work load for each UAV, whereas in \cite{Perez2016} a cell decomposition algorithm based on regular hexagons is proposed for multi-UAV area coverage. In \cite{R1,R2} the coverage path planning problem is posed as a view planning problem \cite{Scott2003}, where the objective is to find the tour of minimum length which allows a UAV equipped with a fixed downward facing camera to inspect a finite set of points on the terrain. Similarly in \cite{R2} a variation of the view planning problem is proposed for solving the coverage planning problem in where the cost to be minimized integrates both the viewing cost and the traveling cost. More recent approaches \cite{Theile2020,Sanna2021} tackle the coverage planning problem with learning based techniques. A deep reinforcement learning approach is proposed \cite{Theile2020} utilizing a single UAV agent for 2D coverage planning, whereas \cite{Sanna2021} proposes a supervised imitation learning based coverage planning approach for multiple UAV agents.
%
%
%
%To summarize, in comparison with the existing CPP approaches, in this work we propose a UAV-based coverage planning technique for 3D environments, which accounts for both the UAV's kinematic and sensing constraints, and thus jointly optimizes the UAV's motion and camera control inputs to obtain optimal coverage trajectories. We integrate ray-tracing into the proposed coverage planning process in order to simulate the physical behavior of light-rays captured by the UAV's camera. This allows us to generate predictive coverage plans over a future planning horizon, and formulate the CPP problem as a rolling finite horizon optimal control problem. Finally, we show that the proposed CPP mathematical formulation can be transformed into a mixed integer program (MIP), and optimally solved with existing optimization tools.
%
%
%
%

TODO









